Ranging-Based Localizability Optimization for Mobile Robotic Networks

In robotic networks relying on noisy range measurements between agents for cooperative localization, the achievable positioning accuracy strongly strongly depends on the network geometry. This motivates the problem of planning robot trajectories in such multi-robot systems in a way that maintains high localization accuracy. We present potential-based planning methods, where localizability potentials are introduced to characterize the quality of the network geometry for cooperative position estimation. These potentials are based on Cramer Rao Lower Bounds (CRLB) and provide a theoretical lower bound on the error covariance achievable by any unbiased position estimator. In the process, we establish connections between CRLBs and the theory of graph rigidity, which has been previously used to plan the motion of robotic networks. We develop decentralized deployment algorithms appropriate for large networks, and we use equality-constrained CRLBs to extend the concept of localizability to scenarios where additional information about the relative positions of the ranging sensors is known. We illustrate the resulting robot deployment methodology through simulated examples and an experiment.

==> parts/macros.tex <==
\newcommand{\der}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dder}[2]{\der{^2 #1}{#2 \partial #2^\top}}
\newcommand{\lder}[2]{\partial #1 / \partial #2 }
\newcommand{\ldder}[2]{\partial^2 #1 / \left(\partial #2 \partial #2^\top \right) }
\newcommand{\lfrac}[2]{ #1 / #2 }

\newcommand{\mbf}{\mathbf}
\renewcommand{\r}{\mathbb{R}}
\newcommand{\esp}[1]{\mathbb{E}\left\{ #1 \right\}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\trace}[1]{\mathrm{Tr}\left\{ #1 \right\}}
\newcommand{\cov}[2]{\mathrm{cov} \left(#1,#2\right)}
\newcommand{\covar}{\mathsf{cov}}
\newcommand{\var}[2]{\mathrm{var} \left(#1\right)}
\newcommand{\condprob}[2]{f\left\{ \left. #1 \right\vert #2 \right\}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\Fu}{\mbf F_\mathcal{U}}

\newcommand{\rk}{\text{rank}}

\newcommand{\col}{\text{col}}

\newcommand{\cpop}[1]{\left[#1\right]_{\times}}

\newcommand{\FOR}{\mathfrak{F}}

\newcommand{\sdim}{n}

\newcommand{\spanv}[1]{\mathrm{span}\left\{ #1 \right\}}
\newcommand{\prov}{{\color{orange} (provisional)}}

\newcommand{\td}[1]{\todo[inline]{JC : #1}}
\newcommand{\jln}[1]{\textcolor{red}{#1}}
\newcommand{\jlnRem}[1]{\textcolor{orange}{#1}}
\newcommand{\jcm}[1]{\textcolor{blue}{#1}}

\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{remark}{Remark}

\newcounter{isdiff}\setcounter{isdiff}{1}

\ifthenelse{\value{isdiff}>0}
{
\newcommand{\diffblock}{\color{blue}}
\newcommand{\diff}[1]{\textcolor{blue}{#1}}
\newcommand{\diffcaption}[1]{\caption{[\diff{New figure}] {\color{blue}#1}}}
}
{
\newcommand{\diffblock}{\color{black}}
\newcommand{\diff}{\textcolor{black}}
\newcommand{\diffcaption}[1]{\caption{#1}}
}
\newcommand{\diffend}{\color{black}}
\newcommand{\rev}[1]{\textcolor{purple}{#1}}


==> parts/proposition-convergence.tex <==
\diffblock
\begin{proposition}
Assume that $J$ and $\mbf f_c$ are twice continuously differentiable, 
and that $(\mbf p^*,\boldsymbol{\lambda}^*)$ is a local-minimum Lagrange multiplier pair 
with a regular point $\mbf p^*$ and that 
$\ldder{(J+(\lambda^*)^\top \mbf f_c)}{\mbf p}\vert_{\mbf p = \mbf p^*} \succ \mbf 0$. 
Then there exists $\bar{\eta}$ such that for all $0< \eta_k \leq \bar{\alpha}$ 
the point $(\mbf p^*,\boldsymbol{\lambda}^*)$ is an attractor of the iterations \eqref{eq:lagrangian_descent}.  
\end{proposition}
\begin{proof}
This proposition is an application of Proposition 5.4.2 in \cite{dimitri_p_bertsekas_nonlinear_2016}.
\end{proof}
\diffend 


==> parts/usecases.tex <==


\section{Simulations}
\label{sec:sim_standard}

In this section, we present two deployment scenarios. The first is a structure 
inspection problem by a multi-robot network maintaining localizability while 
the task is performed. The second concerns the deployment of an Unmanned Ground
Vehicle (UGV) carrying several tags, where we include the distance and relative 
position constraints in the CRLB-based potential.


\subsection{Cooperative Structure Inspection}


Consider $N=5$ mobile robots, where three of them are anchors, i.e., $\mathcal{K} = \{3,4,5\}$, 
assumed to be independently perfectly localized (e.g., via RTK GNSS), and the other two 
are tags, i.e., $\mathcal{U}=\{1,2\}$. 
Each robot carries an UWB transceiver to communicate and take ranging measurements
with any other robot, via Two Way Ranging (TWR) protocol \cite{mai_local_2018,prorok_models_2013}.
The ranging measurements follow the model \eqref{eq:model_meas}.
The tags are required to go underneath an $L\times H := 6~\mathrm{m} \times 10 ~\mathrm{m}$ 
rectangular structure, represented on Fig. \ref{fig:d-opt-traj}, in order to inspect it. 
Once under the structure, the tags lose access to the independent localization
system (e.g., because GNSS signals are blocked).
The anchors' task is then to provide accurate localization for the tags, 
using the algorithms described in this paper.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/D-opt-trajectory.pdf}
    \caption{Trajectories for the cooperative inspection scenario.}
    \label{fig:d-opt-traj}
\end{figure}


\subsubsection{Motion Planner Design}

First, we assume that the tags $\mathcal U = \{1,2\}$ perform the inspection by following 
specified straight paths under the structure, described by the sequences of waypoints 
$\mbf p_{1,l}^d = [L/3,a l]^\top$ and $\mbf p_{2,l}^d = [2L/3,a l]^\top$ with 
$a = 0.1~\mathrm{m}$, $1 \leq l \leq 100$.
The tags follow this path without taking their localization performance 
into account.
On the other hand, the purpose of the mobile anchors is to provide accurate localization 
for the tags, measured here by $J_\text{loc}(\mbf p) = J_D(\mbf p)$ for its 
computational efficiency. Moreover, the anchors must not wander away from the 
tags nor go under the structure, to maintain good localization.
Hence, we introduce a potential 
$J_\text{con}(\mbf p_\mathcal{K}) = \sum_{i\in \mathcal{K}} \sum_{e\in \mathcal{B}_i} g(d(i,e),d_s)$ 
penalizing the anchors if they approach the boundaries of specified bounding boxes $\mathcal{B}_i$,
see Figure \ref{fig:d-opt-traj}.
We use standard repulsive potentials $g(d(i,e),d_s)=0.5(1/d(i,e)-1/d_s)^{2}\mathsf{1}_{d(i,e)<d_s}$,
where $d(i,e)$ is the distance between agent $i$ and edge $e$ of box $\mathcal B_i$,
and $d_s = 1.5~\mathrm{m}$ defines the influence region of the edge \cite{Lynch2017ModernRM}.


Therefore, we define the overall potential for the the anchors as 
$J_\text{anchors}(\mbf p)= K_l J_D(\mbf p) +  K_c J_{con}(\mbf p_\mathcal{K})$ 
where $K_l, K_c>0$ are constant parameters. 
The anchors $i \in \mathcal{K}$ 
implement the \diff{gradient descent} scheme
\begin{equation}
     \mbf p_{i,k+1} = 
     \mbf p_{i,k} - 
     K_l \left( \der{J_D}{\mbf p_{i,k}} \right)^\top 
     - K_c \left( \der{J_\text{con}}{\mbf p_{i,k}} \right)^\top
     \label{eq:simulations:potdesc}
\end{equation}
\diff{with $K_l,K_c > 0$.}
For $\xi_i \in \{x_i,y_i\}$, we compute 
$\partial J_D/\partial \xi_i$
analytically by \eqref{eq:der:Dopt}. 
The expressions of the derivatives $\partial J_\text{con} / \partial {\xi_i}$ of the repulsive potential
are standard \cite{Lynch2017ModernRM}.


The gradient descent scheme is used to obtain desired waypoints
for the anchors, 
which we can track using controllers on the robots.
For concreteness, assume that all robots are identical with \diff{unicycle} kinematics \cite[Chap. 4]{corke_robotics_2011}
\begin{equation}
\dot{x}_M = v\cos(\theta), \quad
\dot{y}_M = v\sin(\theta), \quad
\dot{\theta} = \omega
\label{eq:kine_monocycle}
\end{equation}
where $\omega$ and $v$ are the rotational and transational velocities 
(see Fig \ref{fig:controleptapt}),
$(M,\vec{x}^r,\vec{y}^r)$ is the robot frame and $\theta$ is the robot heading with
respect to $\mathfrak{F}$.
The transceiver's coordinates in the robot frame are
$\mbf p^r = [a,b]^\top$, and we assume that $a \neq 0$. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{figs/controle_pt_a_pt}
	\caption{Robot and anchor trajectory tracking configuration.}
	\label{fig:controleptapt}
\end{figure}


\begin{figure}[b]
	\centering
	\includegraphics[width=0.8\linewidth]{figs/d-opt_with_entropy.pdf}
	\caption{Localizability potential $J_D(\mbf p(k))$ and empirical plot of $\ln \det \mathsf{cov}(\hat{\mbf p}(k))$.}
	\label{fig:d-opt-pot}
\end{figure}

With $\tilde{\mbf u} \in \mathbb R^2$ the coordinates of %tag
the anchor velocity in $\mathfrak{F}$, 
the following Proportional-Integral (PI) controller
\begin{equation}
\tilde{\mbf u} = K_p(\mbf p_d(t) - \mbf p(t)) + K_i \int_{\tau = 0}^t (\mbf p_d(\tau) - \mbf p(\tau))d\tau,
\label{eq:velcontroller}
\end{equation}
for $K_p, K_i >0$, 
allows the anchors to track the desired trajectory $\mbf p_d$. This provides
a velocity command $\mbf u := [v,\omega]^\top$ for the robot,
since $\mbf u = \mbf T (\theta) \tilde{\mbf u}$ \cite[Section 13.3]{Lynch2017ModernRM} with
\[
\mbf T(\theta) =
\frac{1}{a} 
\begin{bmatrix}
a \cos \theta - b \sin \theta & a \sin \theta + b \cos \theta \\
- \sin \theta & 
\cos \theta 
\end{bmatrix}.
\]
\rev{\textbf{add details}}

\subsubsection{Simulation and Performance Analysis}
\label{ss:sim:perf}

We set the initial positions for the tags to 
$\mbf p_{1,0} = [1,-1/2]^\top,\mbf p_{2,0} = [5,-1/2]^\top$
and for the anchors to $\mbf p_{3,0} = [-2,0]^\top,\mbf p_{4,0} = [-1.5,0]^\top,\mbf p_{5,0} = [8,0]^\top$. 
We choose the parameter values in \eqref{eq:simulations:potdesc} as 
$K_l = 2$ and  $K_c = 1/100$. To take into account the physical constraints on the robot velocities, 
we bound the stepsizes $||\mbf p_{i,k+1}-\mbf p_{i,k}||\leq \Delta_\text{vel}$, by
implementing the iterations  
\[
\mbf p_{i,k+1}=\mbf p_{i,k}-\frac{\partial J}{\partial \mbf p_{i,k}} \times 
\min \left\{1,\frac{\Delta_\text{vel}}{||\partial J/\partial \mbf p_{i,k}||}\right \},
\]
\diff{where $J(\mbf p) = K_l J_D(\mbf p)+ K_c K_\text{con}(\mbf p)$}. 
In our simulation, we set $\Delta_{vel} = 0.2~\mathrm{m}$. 
We set $a = 0.5~m$ and $b = 0.5~m$ 
and the PI controller gains are $K_p = 3$, $K_i = 0.5$.
The controller \eqref{eq:velcontroller} follows the trajectory computed 
by \eqref{eq:simulations:potdesc} with a maximum tracking error of about $10$ cm.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/Dopt_mse_montage.pdf}
    \caption{Empirical mean-squared error.}
    \label{fig:d-opt-mse}
\end{figure}

As shown by the trajectories on Fig \ref{fig:d-opt-traj}, the tags 
follow their assigned path and
the anchors maintain the localizability. Initially, all robots are nearly aligned, 
a geometry with poor localizability. As shown on Fig. \ref{fig:d-opt-pot}, 
the anchor deployment quickly and significantly decreases the localizability potential. 
In Fig. \ref{fig:d-opt-mse}, at each iteration $k$ and for each tag $i$, we plot 
the empirical total MSE, i.e., 
$\widetilde{MSE}_{i,k} = \frac{1}{M} \sum_{\rho=1}^M \epsilon_{i,k}^\rho$, 
evaluated via $M$ Monte Carlo simulations 
computing $\epsilon_{i,k}^\rho = ||\hat{\mbf p}_{i,k}^\rho -\mbf p_{i,k}||^2$,
with $\hat{\mbf p}_{i,k}^\rho$ the estimate of $\mbf p_{i,k}$ at simulation $\rho$, 
obtained by solving the least-squares problem
\begin{equation}
\small 
\hat{\mbf p}_{\mathcal{U},k}^\rho = 
\underset{\mbf p_{\mathcal{U}}\in \r^{2 U}}{\text{argmin}} Q(\mbf p_\mathcal{U}) \coloneqq 
\sum_{i\in \mathcal{U}} \sum_{j\in \mathcal N_i} ( \hat{d}_{ij,k}-\tilde{d}_{ij,k}^\rho )^2,
\label{eq:quadratic_cost}
\normalsize
\end{equation}
where $\hat{d}_{ij}:=||\hat{\mbf p}_{i,k} - \hat{\mbf p}_{j,k}||$ 
(with $\hat{\mbf p}_{j,k}$ the anchor position if $j \in \mathcal{K}$)
and $\tilde{d}_{ij,k}^\rho$ the measurements at simulation $\rho$, obtained 
with the Gaussian additive model \eqref{eq:model_meas} for $\sigma = 10~\mathrm{cm}$. 
We simulate $M=500$ realizations and give $3\sigma$ confidence bounds $b_+,b_-$ 
on Fig. \ref{fig:d-opt-mse}. 
These bounds are defined by $b_{\pm,k} = \widetilde{MSE}_{i,k} \pm 3 \widetilde{\sigma}_{i,k}/\sqrt{M}$,
where $\widetilde{\sigma}_{i,k}^2 = \frac{1}{M-1} \sum_{\rho=1}^M [\epsilon_{i,k}^\rho - \widetilde{MSE}_{i,k}]^2$ is the empirical variance of the samples. We remark that the motion planing method improves 
the precision of the estimates significantly during the  first $25$ iterations of motion planning, 
dividing the MSE of tag $1$ by a factor of ten. We plot $\ln \det \tilde{\Sigma}_k$ 
on Fig. \ref{fig:d-opt-pot}, with $\tilde{\Sigma}_k$ the empirical covariance 
of $\hat{\mbf p}_{\mathcal{U},k}$ obtained using \eqref{eq:quadratic_cost}, 
\rev{which shows that localizability as defined by the D-Opt criterion is
properly maintained.} 



